Automatic Model Card Generation Using an LLM

Model cards are structured documents that summarize key information about machine learning models to improve transparency, usability, and accountability. However, they often lack a consistent structure, and many models provide no model cards, making comparison and interpretation difficult. This paper presents two contributions. First, we propose MCTidy, an LLM-based approach that reorganizes existing model cards into a standardized template to improve clarity and comparability. Second, we introduce MCGenie, an LLM-based system that generates model cards directly from model repository data. We apply MCTidy to 48 Hugging Face model cards and evaluate information retention, section alignment, hallucination, and stability. Our findings show high information retention with minimal textual loss, accurate section assignment, rare hallucinations primarily in descriptive sections, and strong stability across runs. We assess MCGenie by generating model cards for the same 48 models and assessing semantic similarity, factual correctness, and sensitivity to input resources. The generated model cards achieved high semantic similarity (mean around 0.9); over half were fully correct, and most remaining errors were minor. Generation quality depended strongly on the availability of supporting resources, particularly associated papers. Overall, our findings demonstrate the potential of LLM-based methods to enable scalable, standardized model card documentation.

==> discussion-generation.tex <==
\subsection{Discussion}
\label{sec:discussion_genration}
Our analysis shows that automated model card generation can capture most of the key information accurately and clearly, but its performance depends heavily on the type and quality of input data. Associated papers are the most important resource, without them, many sections are incomplete or less accurate. Configuration and tokenizer files, though often cited in the generated model cards, have less impact on output quality likely because the papers often contain most of the necessary information. Interestingly, many factual inaccuracies were often linked to misalignment between the model card and cited sources or inconsistencies within the sources themselves, highlighting that errors are as much a reflection of repository data quality. Moreover, from Section~\ref{sec:generationrqresemble}, we see that many (sub)sections which do not contain information in the original (reorganized) model card, also cannot be generated from the repository data, indicating the information for those (sub)sections is not present at all.

For the content similarity measurement in Section~\ref{sec:generationrqresemble}, we considered a cosine similarity score of 0.9 as high degree of semantic similarity, while in Section~\ref{sec:generationrqvaryinginput}, we considered a cosine similarity score of 0.97 or higher as high degree of semantic similarity because in the latter case, we were comparing model cards written by the same author (\generator) and we wanted to identify even the small variations occurred due to changes in input data. Therefore, a higher threshold was needed to indicate that the regenerated card preserved nearly all of the original semantic content without meaningful information loss.

%For future work, integrating retrieval-augmented generation or explicit grounding mechanisms could mitigate errors arising from weak citations and improve consistency across narrative sections, enhancing both transparency and reproducibility. Future work should explore hybrid generation pipelines that explicitly integrate document retrieval and grounding verification to further improve factual robustness and interpretive accuracy in automated documentation systems.

==> fig/_empty_section_comparison_table.tex <==
\begin{tabular}{@{}lrr@{}}
	\toprule
	\textbf{(Sub)sections} & \textbf{Reorganized} & \textbf{Generated} \\
	\midrule
		Model Details/Person or organization developing model & 2.1\% ( 1) & \cellcolor{niceorange!20.833333333333336!white}12.5\% ( 6) \\
		Model Details/Model date & 37.5\% (18) & \cellcolor{softc0!16.666666666666664!white}29.2\% (14) \\
		Model Details/Model version & 10.4\% ( 5) & \cellcolor{softc0!8.333333333333336!white}6.2\% ( 3) \\
		Model Details/Model type & 0.0\% ( 0) & \cellcolor{softc0!0.0!white}0.0\% ( 0) \\
		Model Details/Training details & 4.2\% ( 2) & \cellcolor{softc0!0.0!white}4.2\% ( 2) \\
		Model Details/Paper or other resource for more information & 4.2\% ( 2) & \cellcolor{niceorange!54.16666666666667!white}31.2\% (15) \\
		Model Details/Citation details & 29.2\% (14) & \cellcolor{niceorange!58.333333333333336!white}58.3\% (28) \\
		Model Details/License & 29.2\% (14) & \cellcolor{niceorange!45.833333333333336!white}52.1\% (25) \\
		Model Details/Contact & 56.2\% (27) & \cellcolor{softc0!25.0!white}43.8\% (21) \\
		Intended Use/Primary intended uses & 0.0\% ( 0) & \cellcolor{softc0!0.0!white}0.0\% ( 0) \\
		Intended Use/Primary intended users & 29.2\% (14) & \cellcolor{softc0!4.166666666666671!white}27.1\% (13) \\
		Intended Use/Out-of-scope uses & 39.6\% (19) & \cellcolor{softc0!12.5!white}33.3\% (16) \\
		How to Use & 0.0\% ( 0) & \cellcolor{niceorange!37.5!white}18.8\% ( 9) \\
		Factors/Relevant factors & 31.2\% (15) & \cellcolor{niceorange!8.333333333333343!white}35.4\% (17) \\
		Factors/Evaluation factors & 56.2\% (27) & \cellcolor{softc0!33.33333333333334!white}39.6\% (19) \\
		Metrics/Model performance measures & 14.6\% ( 7) & \cellcolor{niceorange!33.33333333333333!white}31.2\% (15) \\
		Metrics/Decision thresholds & 93.8\% (45) & \cellcolor{softc0!50.0!white}68.8\% (33) \\
		Metrics/Variation approaches & 70.8\% (34) & \cellcolor{softc0!45.83333333333334!white}47.9\% (23) \\
		Evaluation Data/Datasets & 22.9\% (11) & \cellcolor{niceorange!25.000000000000014!white}35.4\% (17) \\
		Evaluation Data/Motivation & 60.4\% (29) & \cellcolor{softc0!33.33333333333333!white}43.8\% (21) \\
		Evaluation Data/Preprocessing & 75.0\% (36) & \cellcolor{softc0!66.66666666666666!white}41.7\% (20) \\
		Training Data/Datasets & 6.2\% ( 3) & \cellcolor{niceorange!58.33333333333334!white}35.4\% (17) \\
		Training Data/Motivation & 35.4\% (17) & \cellcolor{niceorange!16.666666666666657!white}43.8\% (21) \\
		Training Data/Preprocessing & 41.7\% (20) & \cellcolor{softc0!54.16666666666667!white}14.6\% ( 7) \\
		Quantitative Analyses/Unitary results & 29.2\% (14) & \cellcolor{niceorange!25.000000000000007!white}41.7\% (20) \\
		Quantitative Analyses/Intersectional results & 91.7\% (44) & \cellcolor{softc0!12.5!white}85.4\% (41) \\
		Memory or Hardware Requirements/Loading Requirements & 62.5\% (30) & \cellcolor{softc0!50.0!white}37.5\% (18) \\
		Memory or Hardware Requirements/Deploying Requirements & 58.3\% (28) & \cellcolor{niceorange!12.500000000000014!white}64.6\% (31) \\
		Memory or Hardware Requirements/Training or Fine-tuning Requirements & 35.4\% (17) & \cellcolor{niceorange!12.5!white}41.7\% (20) \\
		Ethical Considerations & 27.1\% (13) & \cellcolor{niceorange!8.333333333333336!white}31.2\% (15) \\
		Caveats and Recommendations/Caveats & 6.2\% ( 3) & \cellcolor{niceorange!37.5!white}25.0\% (12) \\
		Caveats and Recommendations/Recommendations & 6.2\% ( 3) & \cellcolor{niceorange!33.33333333333333!white}22.9\% (11) \\
	\bottomrule
\end{tabular}

==> fig/_insufficient_information_comparison_table.tex <==
\begin{tabular}{@{}lrrrr@{}}
	\toprule
	\multirow{2}{*}{\textbf{(Sub)sections}} & \textbf{w All Data} & \textbf{w/o Paper} & \textbf{w/o Config} & \textbf{w/o Tokenizer} \\
	 & (out of 48) & (out of 26) & (out of 46) & (out of 34) \\
	\midrule
		Model Details/Person or organization developing model & 12.5\% ( 6) & \cellcolor{niceorange!29.807692307692307!white}42.3\% (11) & \cellcolor{niceorange!7.065217391304348!white}19.6\% ( 9) & \cellcolor{niceorange!8.088235294117645!white}20.6\% ( 7) \\
		Model Details/Model date & 29.2\% (14) & \cellcolor{niceorange!59.29487179487178!white}88.5\% (23) & \cellcolor{niceorange!3.442028985507246!white}32.6\% (15) & \cellcolor{niceorange!3.186274509803919!white}32.4\% (11) \\
		Model Details/Model version & 6.2\% ( 3) & \cellcolor{niceorange!12.980769230769234!white}19.2\% ( 5) & \cellcolor{niceorange!6.7934782608695645!white}13.0\% ( 6) & 2.9\% ( 1) \\
		Model Details/Model type & 0.0\% ( 0) & 0.0\% ( 0) & 0.0\% ( 0) & 0.0\% ( 0) \\
		Model Details/Training details & 4.2\% ( 2) & 3.8\% ( 1) & \cellcolor{niceorange!21.92028985507246!white}26.1\% (12) & \cellcolor{niceorange!1.715686274509804!white}5.9\% ( 2) \\
		Model Details/Paper or other resource for more information & 31.2\% (15) & \cellcolor{niceorange!41.826923076923066!white}73.1\% (19) & \cellcolor{niceorange!1.358695652173914!white}32.6\% (15) & \cellcolor{niceorange!1.102941176470587!white}32.4\% (11) \\
		Model Details/Citation details & 58.3\% (28) & \cellcolor{niceorange!41.666666666666664!white}100.0\% (26) & \cellcolor{niceorange!2.536231884057976!white}60.9\% (28) & 55.9\% (19) \\
		Model Details/License & 52.1\% (25) & \cellcolor{niceorange!20.99358974358973!white}73.1\% (19) & \cellcolor{niceorange!4.438405797101446!white}56.5\% (26) & \cellcolor{niceorange!9.681372549019606!white}61.8\% (21) \\
		Model Details/Contact & 43.8\% (21) & \cellcolor{niceorange!44.71153846153845!white}88.5\% (23) & 41.3\% (19) & \cellcolor{niceorange!6.25!white}50.0\% (17) \\
		Intended Use/Primary intended uses & 0.0\% ( 0) & 0.0\% ( 0) & \cellcolor{niceorange!8.695652173913043!white}8.7\% ( 4) & 0.0\% ( 0) \\
		Intended Use/Primary intended users & 27.1\% (13) & \cellcolor{niceorange!49.839743589743605!white}76.9\% (20) & \cellcolor{niceorange!5.525362318840582!white}32.6\% (15) & \cellcolor{niceorange!11.151960784313726!white}38.2\% (13) \\
		Intended Use/Out-of-scope uses & 33.3\% (16) & \cellcolor{niceorange!39.74358974358974!white}73.1\% (19) & \cellcolor{niceorange!10.14492753623189!white}43.5\% (20) & \cellcolor{niceorange!13.725490196078432!white}47.1\% (16) \\
		How to Use & 18.8\% ( 9) & \cellcolor{niceorange!23.557692307692307!white}42.3\% (11) & \cellcolor{niceorange!2.9891304347826093!white}21.7\% (10) & \cellcolor{niceorange!4.7794117647058805!white}23.5\% ( 8) \\
		Factors/Relevant factors & 35.4\% (17) & \cellcolor{niceorange!45.3525641025641!white}80.8\% (21) & \cellcolor{niceorange!5.887681159420282!white}41.3\% (19) & \cellcolor{niceorange!8.700980392156858!white}44.1\% (15) \\
		Factors/Evaluation factors & 39.6\% (19) & \cellcolor{niceorange!48.878205128205124!white}88.5\% (23) & \cellcolor{niceorange!1.7210144927536248!white}41.3\% (19) & \cellcolor{niceorange!7.475490196078432!white}47.1\% (16) \\
		Metrics/Model performance measures & 31.2\% (15) & \cellcolor{niceorange!49.519230769230774!white}80.8\% (21) & 30.4\% (14) & \cellcolor{niceorange!4.044117647058826!white}35.3\% (12) \\
		Metrics/Decision thresholds & 68.8\% (33) & \cellcolor{niceorange!23.557692307692307!white}92.3\% (24) & \cellcolor{niceorange!2.9891304347826093!white}71.7\% (33) & \cellcolor{niceorange!10.661764705882348!white}79.4\% (27) \\
		Metrics/Variation approaches & 47.9\% (23) & \cellcolor{niceorange!48.23717948717949!white}96.2\% (25) & 47.8\% (22) & 47.1\% (16) \\
		Evaluation Data/Datasets & 35.4\% (17) & \cellcolor{niceorange!53.04487179487178!white}88.5\% (23) & 34.8\% (16) & \cellcolor{niceorange!8.700980392156858!white}44.1\% (15) \\
		Evaluation Data/Motivation & 43.8\% (21) & \cellcolor{niceorange!52.40384615384616!white}96.2\% (25) & 43.5\% (20) & \cellcolor{niceorange!6.25!white}50.0\% (17) \\
		Evaluation Data/Preprocessing & 41.7\% (20) & \cellcolor{niceorange!46.79487179487178!white}88.5\% (23) & \cellcolor{niceorange!1.8115942028985472!white}43.5\% (20) & \cellcolor{niceorange!5.3921568627450895!white}47.1\% (16) \\
		Training Data/Datasets & 35.4\% (17) & \cellcolor{niceorange!29.967948717948715!white}65.4\% (17) & \cellcolor{niceorange!3.713768115942024!white}39.1\% (18) & \cellcolor{niceorange!5.7598039215686185!white}41.2\% (14) \\
		Training Data/Motivation & 43.8\% (21) & \cellcolor{niceorange!56.25!white}100.0\% (26) & 41.3\% (19) & \cellcolor{niceorange!6.25!white}50.0\% (17) \\
		Training Data/Preprocessing & 14.6\% ( 7) & \cellcolor{niceorange!0.8012820512820511!white}15.4\% ( 4) & \cellcolor{niceorange!2.807971014492752!white}17.4\% ( 8) & \cellcolor{niceorange!20.71078431372549!white}35.3\% (12) \\
		Quantitative Analyses/Unitary results & 41.7\% (20) & \cellcolor{niceorange!46.79487179487178!white}88.5\% (23) & 37.0\% (17) & \cellcolor{niceorange!2.4509803921568576!white}44.1\% (15) \\
		Quantitative Analyses/Intersectional results & 85.4\% (41) & \cellcolor{niceorange!14.583333333333343!white}100.0\% (26) & 82.6\% (38) & 82.4\% (28) \\
		Memory or Hardware Requirements/Loading Requirements & 37.5\% (18) & \cellcolor{niceorange!12.5!white}50.0\% (13) & \cellcolor{niceorange!16.847826086956516!white}54.3\% (25) & \cellcolor{niceorange!6.617647058823529!white}44.1\% (15) \\
		Memory or Hardware Requirements/Deploying Requirements & 64.6\% (31) & \cellcolor{niceorange!27.724358974358964!white}92.3\% (24) & \cellcolor{niceorange!2.8079710144927503!white}67.4\% (31) & \cellcolor{niceorange!6.004901960784309!white}70.6\% (24) \\
		Memory or Hardware Requirements/Training or Fine-tuning Requirements & 41.7\% (20) & \cellcolor{niceorange!39.1025641025641!white}80.8\% (21) & 41.3\% (19) & 41.2\% (14) \\
		Ethical Considerations & 31.2\% (15) & \cellcolor{niceorange!37.980769230769226!white}69.2\% (18) & \cellcolor{niceorange!3.532608695652172!white}34.8\% (16) & \cellcolor{niceorange!9.92647058823529!white}41.2\% (14) \\
		Caveats and Recommendations/Caveats & 25.0\% (12) & \cellcolor{niceorange!28.846153846153847!white}53.8\% (14) & 17.4\% ( 8) & \cellcolor{niceorange!1.4705882352941195!white}26.5\% ( 9) \\
		Caveats and Recommendations/Recommendations & 22.9\% (11) & \cellcolor{niceorange!54.00641025641027!white}76.9\% (20) & 21.7\% (10) & \cellcolor{niceorange!9.436274509803923!white}32.4\% (11) \\
	\bottomrule
\end{tabular}
